In the Saddle: Chasing Fast and Repeatable Features

A novel similarity-covariant feature detector that extracts points whose neighbourhoods, when treated as a 3D intensity surface, have a saddle-like intensity profile. The saddle condition is verified efficiently by intensity comparisons on two concentric rings that must have exactly two dark-to-bright and two bright-to-dark transitions satisfying certain geometric constraints. Experiments show that the Saddle features are general, evenly spread and appearing in high density in a range of images. The Saddle detector is among the fastest proposed. In comparison with detector with similar speed, the Saddle features show superior matching performance on number of challenging datasets.

==> figures/inlier-coverage.tex <==
%% Inlier in yellow dots and coverage footprints
\begin{figure*}
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%
\parbox{.12\linewidth}{\centering \fbox{\includegraphics[width=0.99\linewidth]{images/ICenters_Light_pair_2_dct_saddle}}\\\fbox{\includegraphics[width=0.99\linewidth]{images/IMask_Light_pair_2_dct_saddle}}\\\dt\\($75\%$)}
\parbox{.12\linewidth}{\centering \fbox{\includegraphics[width=0.99\linewidth]{images/ICenters_Light_pair_2_dct_fast}}\\\fbox{\includegraphics[width=0.99\linewidth]{images/IMask_Light_pair_2_dct_fast}}\\ORB\\($45\%$)}
\parbox{.12\linewidth}{\centering \fbox{\includegraphics[width=0.99\linewidth]{images/ICenters_Light_pair_2_dct_surf}}\\\fbox{\includegraphics[width=0.99\linewidth]{images/IMask_Light_pair_2_dct_surf}}\\SURF\\($53\%$)}
\parbox{.12\linewidth}{\centering \fbox{\includegraphics[width=0.99\linewidth]{images/ICenters_Light_pair_2_dct_sift}}\\\fbox{\includegraphics[width=0.99\linewidth]{images/IMask_Light_pair_2_dct_sift}}\\DoG\\($57\%$)}
\parbox{.12\linewidth}{\centering \fbox{\includegraphics[width=0.99\linewidth]{images/Dots_Bark_pair1Threshold_iterator1_Detector_saddle}}\\\fbox{\includegraphics[width=0.99\linewidth]{images/Mask_Barkpair1_Threshold_iterator1Detectorsaddle}}\\ \dt\\($66\%$)}
\parbox{.12\linewidth}{\centering \fbox{\includegraphics[width=0.99\linewidth]{images/Dots_Bark_pair1Threshold_iterator1_Detector_fast}}\\\fbox{\includegraphics[width=0.99\linewidth]{images/Mask_Barkpair1_Threshold_iterator1Detectorfast}}\\ ORB\\ ($45\%$)}
\parbox{.12\linewidth}{\centering \fbox{\includegraphics[width=0.99\linewidth]{images/Dots_Bark_pair1Threshold_iterator1_Detector_surf}}\\\fbox{\includegraphics[width=0.99\linewidth]{images/Mask_Barkpair1_Threshold_iterator1Detectorsurf}}\\ SURF\\ ($59\%$)}
\parbox{.12\linewidth}{\centering \fbox{\includegraphics[width=0.99\linewidth]{images/Dots_Bark_pair1Threshold_iterator1_Detector_sift}}\\\fbox{\includegraphics[width=0.99\linewidth]{images/Mask_Barkpair1_Threshold_iterator1Detectorsift}}\\ DoG\\ ($40\%$)}


\caption{Coverage by ground-truth validated feature matches  on selected image pairs from the Oxford dataset\cite{Mikolajczyk2005,Mikolajczyk2005a}. Yellow dots mark positions of the features (top). The covered area is computed as a union of circles with a 25 pixel radius centered on the matches(bottom).}
\label{fig.coverage}
\end{figure*}

==> figures/inner-outer-template.tex <==
%%%%% Figure. Inner and outer template window
\begin{figure}
\centering
\setlength{\fboxsep}{0pt}%
\parbox{.45\linewidth}{\centering \fbox{\begin{overpic}[width=\linewidth]{images/Templates}
% Center
\put (47,47) {\small$p$}
% Outer
\put (46,6) {\small$b_1$}
\put (59,6) {\small$b_2$}
\put (29,6) {\small$b_{16}$}

\put (74,19) {\small$b_3$}
\put (74,74) {\small$b_7$}
\put (17,74) {\small$b_{11}$}
\put (17,19) {\small$b_{15}$}

\put (88,34) {\small$b_4$}
\put (88,46) {\small$b_5$}
\put (88,60) {\small$b_6$}

\put (46,88) {\small$b_9$}
\put (60,88) {\small$b_8$}
\put (31,88) {\small$b_{10}$}

\put (3,34) {\small$b_{14}$}
\put (3,46) {\small$b_{13}$}
\put (3,60) {\small$b_{12}$}

% Inner
\comment{
\put (46,33) {\small$a_1$}
\put (60,33) {\small$a_2$}
\put (32,46) {\small$a_7$}
\put (32,33) {\small$a_8$}

\put (46,60) {\small$a_5$}
\put (60,46) {\small$a_3$}
\put (60,60) {\small$a_4$}
\put (32,60) {\small$a_6$}
}

\end{overpic}}}
\parbox{.23\linewidth}{\centering \fbox{\includegraphics[width=0.95\linewidth]{images/TemplCase1}}\vspace{1pt}\\\fbox{\includegraphics[width=0.95\linewidth]{images/TemplCase8}}}
\parbox{.23\linewidth}{\centering \fbox{\includegraphics[width=0.95\linewidth]{images/TemplCase5}}\vspace{1pt}\\\fbox{\includegraphics[width=0.95\linewidth]{images/TemplCase2}}}

\caption{The 8 pixel positions marked in red form the \textit{inner ring} and the 16 positions $b_j$ in blue form the \textit{outer ring}. Positions shared by both rings are bicolored.}
\label{fig:innerouter}
\end{figure}
% The second and third columns depict example of accepted patterns.






==> tables/matching-table-fast.tex <==
\begin{table*}[tb]
\centering
\caption{Matching algorithm comparison in fast setups with BRIEF descriptor. The subcolumns are: number of matched image pairs (left),average running time(all stages - read image-detect-describe-match-ransac), average number of inliers in matched pairs.  The datasets are listed in Table~\ref{tab:all-datasets}}
\label{tab:matching-fast}
\small
\setlength{\tabcolsep}{.25em}
\vspace{0.5em}
\begin{tabular}{|l|r|l|rrr|rrr|rrr|}
\hline
Alg.
&Sens
&Desc
& \multicolumn{3}{c|}{EF}
& \multicolumn{3}{c|}{OxAff}
& \multicolumn{3}{c|}{SymB}
\\
&&& \shortstack{33 \\\#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#}
& \shortstack{40\\\#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#}
& \shortstack{46\\\#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#}
\\\#} 
\\
\hline
Saddle&500&BRIEF & \ccaEF{2} & 0.3 & 32 & \ccaoxford{22} & 0.3 & 47 & \ccasymbench{1} & 0.3 & 41\\
Saddle&500&FREAK & \ccaEF{11} & 0.3 & 29 & \ccaoxford{26} & 0.4 & 77 & \ccasymbench{8} & 0.4 & 32\\
ORB&500&BRIEF & \ccaEF{16} & 0.1 & 28 & \ccaoxford{27} & 0.1 & 110 & \ccasymbench{14} & 0.2 & 30\\
ORB&500&FREAK & \ccaEF{0} & 0.1 & 0 & \ccaoxford{0} & 0.5 & 0 & \ccasymbench{0} & 0.2 & 0\\
\hline
Saddle&1000&BRIEF & \ccaEF{2} & 0.3 & 52 & \ccaoxford{25} & 0.3 & 92 & \ccasymbench{3} & 0.3 & 70\\
Saddle&1000&FREAK & \ccaEF{14} & 0.4 & 47 & \ccaoxford{29} & 0.4 & 145 & \ccasymbench{11} & 0.4 & 59\\
ORB&1000&BRIEF & \ccaEF{18} & 0.2 & 52 & \ccaoxford{28} & 0.2 & 208 & \ccasymbench{21} & 0.2 & 51\\
ORB&1000&FREAK & \ccaEF{0} & 0.2 & 0 & \ccaoxford{0} & 0.3 & 0 & \ccasymbench{0} & 0.2 & 0\\
\hline
Saddle+ORB&500&BRIEF & \ccaEF{7} & 0.3 & 51 & \ccaoxford{27} & 0.4 & 140 & \ccasymbench{11} & 0.4 & 41\\
Saddle+ORB&500&FREAK & \ccaEF{19} & 0.4 & 42 & \ccaoxford{29} & 0.6 & 170 & \ccasymbench{14} & 0.5 & 51\\
\hline
Saddle+ORB&1000&BRIEF & \ccaEF{9} & 0.3 & 75 & \ccaoxford{28} & 0.4 & 269 & \ccasymbench{12} & 0.4 & 82\\
Saddle+ORB&1000&FREAK & \ccaEF{18} & 0.4 & 87 & \ccaoxford{31} & 0.9 & 317 & \ccasymbench{21} & 0.5 & 85\\

\hline
\end{tabular}
\end{table*}

==> tables/matching-table.tex <==
\begin{table*}[tb]
\centering
\caption{Matching algorithm comparison in slow setup with combination of RootSIFT and HalfRootSIFT descriptors. The subcolumns are: number of matched image pairs (left),average running time (all stages - read image-detect-describe-match-ransac), average number of inliers in matched pairs.  NMS stands for spatial non-maximum supression. The datasets are listed in Table~\ref{tab:all-datasets}. Most time is taken for description and matching.}
\label{tab:matching}
\small
\setlength{\tabcolsep}{.25em}
\vspace{0.5em}
\begin{tabular}{|l|r|l|rrr|rrr|rrr|rrr|rrr|rrr|}
\hline
Alg.
&Sens
&\begin{turn}{90}NMS\end{turn}
& \multicolumn{3}{c|}{EF}
& \multicolumn{3}{c|}{LostInPast}
& \multicolumn{3}{c|}{OxAff}
& \multicolumn{3}{c|}{GDB}
& \multicolumn{3}{c|}{SymB}
& \multicolumn{3}{c|}{EVD}
\\
&&& \shortstack{33 \\\#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#}
& \shortstack{172\\\#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#} 
& \shortstack{40\\\#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#}
& \shortstack{46\\\#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#}
& \shortstack{22\\\#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#} 
& \shortstack{15\\ \#}& \shortstack{time \\ $[s]$}& \shortstack{inl \\\#} 
\\
\hline
Saddle&500&- & \ccaEF{18} & 0.9 & 30 & \ccalostinpast{3} & 1.0 & 32 & \ccaoxford{32} & 1.1 & 120 & \ccasnavely{15} & 1.0 & 39 & \ccastewart{7} & 1.1 & 49 & \ccaEVD{0} & 1.0 & 0\\
ORB&500&- & \ccaEF{6} & 1.3 & 27 & \ccalostinpast{2} & 1.2 & 21 & \ccaoxford{31} & 1.4 & 82 & \ccasnavely{7} & 1.3 & 38 & \ccastewart{5} & 1.4 & 26 & \ccaEVD{0} & 1.4 & 0\\
\hline
Saddle&500&+ & \ccaEF{22} & 1.0 & 38 & \ccalostinpast{8} & 1.0 & 27 & \ccaoxford{33} & 1.1 & 160 & \ccasnavely{17} & 1.1 & 54 & \ccastewart{11} & 1.1 & 55 & \ccaEVD{0} & 1.0 & 0\\
ORB&500&+ & \ccaEF{12} & 1.4 & 37 & \ccalostinpast{12} & 1.4 & 22 & \ccaoxford{36} & 1.5 & 112 & \ccasnavely{12} & 1.4 & 46 & \ccastewart{6} & 1.6 & 70 & \ccaEVD{0} & 1.5 & 0\\
\hline
Saddle&1000&- & \ccaEF{25} & 1.7 & 44 & \ccalostinpast{15} & 1.8 & 26 & \ccaoxford{33} & 1.9 & 227 & \ccasnavely{25} & 2.0 & 58 & \ccastewart{12} & 2.0 & 65 & \ccaEVD{0} & 1.7 & 0\\
ORB&1000&- & \ccaEF{15} & 2.4 & 41 &  \ccalostinpast{10} & 2.5 & 31 & \ccaoxford{33} & 2.7 & 143 & \ccasnavely{19} & 2.3 & 44 & \ccastewart{7} & 2.5 & 51 & \ccaEVD{0} & 2.6 & 0\\
\hline
Saddle&1000&+ & \ccaEF{28} & 1.6 & 61 & \ccalostinpast{25} & 1.8 & 31 & \ccaoxford{33} & 1.9 & 315 & \ccasnavely{29} & 1.9 & 76 & \ccastewart{15} & 1.8 & 87 & \ccaEVD{0} & 1.8 & 0\\
ORB&1000&+ & \ccaEF{24} & 2.5 & 49 & \ccalostinpast{16} & 2.4 & 33 & \ccaoxford{37} & 2.6 & 222 & \ccasnavely{27} & 2.4 & 55 & \ccastewart{12} & 2.4 & 83 & \ccaEVD{0} & 2.5 & 0\\
\hline
SURF&default&+& \ccaEF{31} & 1.0 & 52 & \ccalostinpast{17} & 1.3 & 32 & \ccaoxford{37} & 2.3 & 483 & \ccasnavely{34} & 2.0 & 95 & \ccastewart{16} & 2.1 & 97 & \ccaEVD{0} & 1.6 & 0\\
Hess &$\theta=5.3$ &+&\ccaEF{33} & 3.0 & 126 & \ccalostinpast{43} & 3.9 & 40 & \ccaoxford{39} & 8.3 & 1206 & \ccasnavely{39} & 5.9 & 215 & \ccastewart{19} & 8.4 & 238 & \ccaEVD{1} & 5.3 & 22\\
HessAf &$\theta=5.3$ &+&\ccaEF{33} & 3.0 & 85 & \ccalostinpast{27} & 3.6 & 34 & \ccaoxford{40} & 7.6 & 983 & \ccasnavely{35} & 5.2 & 158 & \ccastewart{19} & 8.1 & 189 & \ccaEVD{3} & 4.2 & 25\\
\hline
MODS & &&\ccaEF{33} & 3.5 & 29 & \ccalostinpast{76} & 21 & 20 & \ccaoxford{40} & 1.3 & 102 & \ccasnavely{42} & 10 & 27 & \ccastewart{18} & 10 & 45 & \cellcolor{black}\color{white}{15} & 14 & 27\\
MODS-Saddle & &&\ccaEF{33} & 5.8 & 38 & \ccalostinpast{76} & 25 & 30 & \ccaoxford{40} & 2.2 & 115 & \ccasnavely{38} & 17 & 58 & \ccastewart{18} & 13 & 117 & \cellcolor{black}\color{white}{15} & 23 & 111\\
WXBS&& & \ccaEF{33} & 1.8 & 40 & \cellcolor{black}\color{white}{107} & 42 & 22 & \ccaoxford{40} & 1.9 & 147 & \ccasnavely{45} & 9.4 & 45 & \ccastewart{22} & 7.8 & 92 & \cellcolor{black}\color{white}{15} & 8.5 & 43\\
\hline
\end{tabular}
\end{table*}

